Dark Energy Survey Year 1 Results: Cross-correlation between DES Y1 galaxy weak lensing and SPT+Planck CMB weak lensing

We cross-correlate galaxy weak lensing measurements from the Dark Energy Survey (DES) year-one (Y1) data with a cosmic microwave background (CMB) weak lensing map derived from South Pole Telescope (SPT) and Planck data, with an effective overlapping area of 1289 deg$^{2}$. With the combined measurements from four source galaxy redshift bins, we reject the hypothesis of no lensing with a significance of $10.8\sigma$. When employing angular scale cuts, this significance is reduced to $6.8\sigma$, which remains the highest signal-to-noise measurement of its kind to date. We fit the amplitude of the correlation functions while fixing the cosmological parameters to a fiducial $\Lambda$CDM model, finding $A = 0.99 \pm 0.17$. We additionally use the correlation function measurements to constrain shear calibration bias, obtaining constraints that are consistent with previous DES analyses. Finally, when performing a cosmological analysis under the $\Lambda$CDM model, we obtain the marginalized constraints of $\Omega_{\rm m}=0.261^{+0.070}_{-0.051}$ and $S_{8}\equiv \sigma_{8}\sqrt{\Omega_{\rm m}/0.3} = 0.660^{+0.085}_{-0.100}$. These measurements are used in a companion work that presents cosmological constraints from the joint analysis of two-point functions among galaxies, galaxy shears, and CMB lensing using DES, SPT and Planck data.

==> affil2.tex <==
\section{Affiliations}
%\textit{
$^{1}$ Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, 452 Lomita Mall, Stanford, CA 94305\\ 
$^{2}$ Dept. of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305\\ 
$^{3}$ Department of Physics and McGill Space Institute, McGill University, Montreal, Quebec H3A 2T8, Canada\\ 
$^{4}$ Center for Particle Cosmology, Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA,  USA 19104\\ 
$^{5}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL, USA 60637\\ 
$^{6}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\ 
$^{7}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08193 Barcelona, Spain\\ 
$^{8}$ High Energy Physics Division, Argonne National Laboratory, Argonne, IL, USA 60439\\ 
$^{9}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL, USA 60637\\ 
$^{10}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University,Columbus, OH 43210, USA\\ 
$^{11}$ Department of Physics and Astronomy, McMaster University, 1280 Main St. W., Hamilton, ON L8S 4L8, Canada\\ 
$^{12}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL, USA 60637\\ 
$^{13}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\ 
$^{14}$ Fermi National Accelerator Laboratory, MS209, P.O. Box 500, Batavia, IL 60510\\ 
$^{15}$ Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721\\ 
$^{16}$ Jet Propulsion Laboratory, California Institute of Technology, Pasadena, CA 91109, USA\\ 
$^{17}$ Max-Planck-Institut f\"{u}r extraterrestrische Physik, 85748 Garching, Germany\\ 
$^{18}$ Faculty of Physics, Ludwig-Maximilians-Universit\"{a}t, 81679 M\"{u}nchen, Germany\\ 
$^{19}$ Institut de F\'{i}sica d`Altes Energies (IFAE), The Barcelona Instituteof Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\ 
$^{20}$ Universit\"{a}ts-Sternwarte, Fakult\"{a}t f\"{u}r Physik, Ludwig Maximilians Universit\"{a}t M\"{u}nchen, Scheinerstr. 1, 81679 M\"{u}nchen, Germany\\ 
$^{21}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\ 
$^{22}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\ 
$^{23}$ Einstein Fellow\\ 
$^{24}$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\ 
$^{25}$ Astronomy Department, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\ 
$^{26}$ Department of Physics, University of Illinois Urbana-Champaign, 1110 W. Green Street, Urbana, IL 61801, USA\\ 
$^{27}$ Canadian Institute for Advanced Research, CIFAR Program in Cosmology and Gravity, Toronto, ON, M5G 1Z8, Canada\\ 
$^{28}$ Department of Physics, University of Michigan, Ann  Arbor, MI, USA 48109\\ 
$^{29}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\ 
$^{30}$ Instituci\'{o} Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\ 
$^{31}$ School of Physics, University of Melbourne, Parkville, VIC 3010, Australia\\ 
$^{32}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973,USA\\ 
$^{33}$ Centro de Investigaciones Energ\'{e}ticas, Medioambientales y Tecnol\'{o}ogicas(CIEMAT), Madrid, Spain\\ 
$^{34}$ SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, CA 94025\\ 
$^{35}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\ 
$^{36}$ Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile\\ 
$^{37}$ Department of Physics and Electronics, Rhodes University, PO Box 94, Grahamstown, 6140, South Africa\\ 
$^{38}$ Institute of Cosmology \& Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\ 
$^{39}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\ 
$^{40}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\ 
$^{41}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\ 
$^{42}$ Department of Physics, University of Chicago, Chicago, IL, USA 60637\\ 
$^{43}$ Enrico Fermi Institute, University of Chicago, Chicago, IL, USA 60637\\ 
$^{44}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\ 
$^{45}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\ 
$^{46}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\ 
$^{47}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\ 
$^{48}$ California Institute of Technology, Pasadena, CA, USA 91125\\ 
$^{49}$ Department of Physics, University of California, Berkeley, CA, USA 94720\\ 
$^{50}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\ 
$^{51}$ Excellence Cluster Universe, 85748 Garching, Germany\\ 
$^{52}$ Center for Astrophysics and Space Astronomy, Department of Astrophysical and Planetary Sciences, University of Colorado, Boulder, CO, 80309\\ 
$^{53}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\ 
$^{54}$ European Southern Observatory, Karl-Schwarzschild-Stra{\ss}e 2, 85748 Garching, Germany\\ 
$^{55}$ Department of Physics, University of Colorado, Boulder, CO, 80309\\ 
$^{56}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\ 
$^{57}$ University of Chicago, Chicago, IL, USA 60637\\ 
$^{58}$ Harvard-Smithsonian Center for Astrophysics, Cambridge, MA, USA 02138\\ 
$^{59}$ Australian Astronomical Observatory, North Ryde, NSW 2113, Australia\\ 
$^{60}$ Departamento de F\'{i}sica Matem\'{a}tica, Instituto de F\'{i}sica, Universidade de Sa\~{o} Paulo, CP 66318, Sa\~{o} Paulo, SP, 05314-970, Brazil\\ 
$^{61}$ Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA, USA 94720\\ 
$^{62}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\ 
$^{63}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\ 
$^{64}$ Dunlap Institute for Astronomy \& Astrophysics, University of Toronto, 50 St George St, Toronto, ON, M5S 3H4, Canada\\ 
$^{65}$ Department of Physics, University of Minnesota, Minneapolis, MN, USA 55455\\ 
$^{66}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\ 
$^{67}$ Physics Department, Center for Education and Research in Cosmology and Astrophysics, Case Western Reserve University,Cleveland, OH, USA 44106\\ 
$^{68}$ Liberal Arts Department, School of the Art Institute of Chicago, Chicago, IL, USA 60603\\ 
$^{69}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\ 
$^{70}$ Brandeis University, Physics Department, 415 South Street, Waltham MA 02453\\ 
$^{71}$ Instituto de F\'{i}sica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil\\ 
$^{72}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\ 
$^{73}$ Department of Astronomy \& Astrophysics, University of Toronto, 50 St George St, Toronto, ON, M5S 3H4, Canada\\ 
$^{74}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\ 
%}

==> authlistbackup.tex <==
%\author[T. Giannantonio, P. Fosalba et al.] {T.~Giannantonio$^{1,2,3}$\thanks{t.giannantonio@ast.cam.ac.uk}, P.~Fosalba$^{4 \thanks{fosalba@ice.cat}}$,
%B. Hoyle, D. Gruen, G. M. Bernstein, M. M. Rau, J. De Vicente, W. G. Hartley, E. Gaztanaga, J. DeRose, M. A. Troxel, C. Davis, A. Alarcon, N. MacCrann, J. Prat, C. Sánchez, E. Sheldon, R. H. Wechsler,
\def\KIPAC{1}
\def\Stanford{2}
\def\McGill{3}
\def\Penn{4}
\def\KICP{5}
\def\UCL{6}
\def\IEEC{7}
\def\ArgonneHEP{8}
\def\KICPChicago{9}
\def\CCAPP{10}
\def\McMaster{11}
\def\AAUChicago{12}
\def\CMU{13}
\def\FNAL{14}
\def\Arizona{15}
\def\JPL{16}
\def\MPE{17}
\def\Munich{18}
\def\IFAE{19}
\def\LMU{20}
\def\KICC{21}
\def\IoA{22}
\def\Einstein{23}
\def\ETH{24}
\def\Illast{25}
\def\Illphys{26}
\def\Cifar{27}
\def\Michigan{28}
\def\OSU{29}
\def\ICREA{30}
\def\Melbourne{31}
\def\BNL{32}
\def\CIEMAT{33}
\def\SLAC{34}
\def\Edinburgh{35}
\def\CTIO{36}
\def\Rhodes{37}
\def\Portsmouth{38}
\def\CNRS{39}
\def\Sorbonne{40}
\def\Manchester{41}
\def\PhysicsUChicago{42}
\def\EFIChicago{43}
\def\LIneA{44}
\def\ONR{45}
\def\NCSA{46}
\def\ICE{47}
\def\Caltech{48}
\def\Berkeley{49}
\def\IITHyderabad{50}
\def\ExcellenceCluster{51}
\def\Colorado{52}
\def\UAM{53}
\def\ESO{54}
\def\Colphys{55}
\def\SCIPP{56}
\def\UChicago{57}
\def\CfA{58}
\def\AAO{59}
\def\SaoPaulo{60}
\def\LBNL{61}
\def\TAMU{62}
\def\Princeton{63}
\def\Dunlap{64}
\def\Minnesota{65}
\def\Sussex{66}
\def\CaseWestern{67}
\def\ArtInstChicago{68}
\def\Southampton{69}
\def\Brandeis{70}
\def\IFGW{71}
\def\ORNL{72}
\def\UToronto{73}
\def\ANL{74}

\author[Omori et al.] {
\parbox{\textwidth}{
\normalsize Y.~Omori$^{\KIPAC,\Stanford,\McGill}$,
E.~Baxter$^{\Penn}$,
C.~Chang$^{\KICP}$,
D.~Kirk$^{\UCL}$,
A.~Alarcon$^{\IEEC}$,
G.~M.~Bernstein$^{\Penn}$,
L.~E.~Bleem$^{\ArgonneHEP,\KICPChicago}$,
R.~Cawthon$^{\KICP}$,
A.~Choi$^{\CCAPP}$,
R.~Chown$^{\McGill,\McMaster}$,
T.~M.~Crawford$^{\KICPChicago,\AAUChicago}$,
C.~Davis$^{\KIPAC}$,
J.~DeRose$^{\KIPAC,\Stanford}$,
S.~Dodelson$^{\CMU,\FNAL}$,
T.~F.~Eifler$^{\Arizona,\JPL}$,
P.~Fosalba$^{\IEEC}$,
O.~Friedrich$^{\MPE,\Munich}$,
M.~Gatti$^{\IFAE}$,
E.~Gaztanaga$^{\IEEC}$,
T.~Giannantonio$^{\LMU,\KICC,\IoA}$,
D.~Gruen$^{\KIPAC,\Stanford,\Einstein}$,
W.~G.~Hartley$^{\UCL,\ETH}$
G.~P.~Holder$^{\Illast,\Illphys,\Cifar}$,
B.~Hoyle$^{\LMU}$,
D.~Huterer$^{\Michigan}$,
B.~Jain$^{\Penn}$,
M.~Jarvis$^{\Penn}$,
E.~Krause$^{\Arizona,\JPL}$,
N.~MacCrann$^{\CCAPP,\OSU}$,
R.~Miquel$^{\IFAE,\ICREA}$,
J.~Prat$^{\IFAE}$,
M.~M.~Rau$^{\LMU}$,
C.~L.~Reichardt$^{\Melbourne}$,
E.~Rozo$^{\Arizona}$,
S.~Samuroff$^{\CMU}$,
C.~S{\'a}nchez$^{\Penn}$,
L.~F.~Secco$^{\Penn}$,
E.~Sheldon$^{\BNL}$,
G.~Simard$^{\McGill}$,
M.~A.~Troxel$^{\CCAPP,\OSU}$,
J.~De~Vicente$^{\CIEMAT}$,
P.~Vielzeuf$^{\IFAE}$,
R.~H.~Wechsler$^{\KIPAC,\Stanford,\SLAC}$,
J.~Zuntz$^{\Edinburgh}$,
T.~M.~C.~Abbott$^{\CTIO}$,
F.~B.~Abdalla$^{\UCL,\Rhodes}$,
S.~Allam$^{\FNAL}$,
J.~Annis$^{\FNAL}$,
S.~Avila$^{\Portsmouth}$,
E.~Bertin$^{\CNRS,\Sorbonne}$,
S.~L.~Bridle$^{\Manchester}$,
D.~Brooks$^{\UCL}$,
D.~L.~Burke$^{\KIPAC,\SLAC}$,
J.~E.~Carlstrom$^{\KICPChicago,\PhysicsUChicago,\ArgonneHEP,\AAUChicago,\EFIChicago}$,
A.~Carnero~Rosell$^{\LIneA,\ONR}$,
M.~Carrasco~Kind$^{\Illast,\NCSA}$,
J.~Carretero$^{\IFAE}$,
F.~J.~Castander$^{\IEEC,\ICE}$,
C.~L.~Chang$^{\ArgonneHEP,\KICPChicago,\AAUChicago}$,
H-M.~Cho$^{\SLAC}$,
A.~T.~Crites$^{\KICPChicago,\AAUChicago,\Caltech}$,
M.~Crocce$^{\IEEC,\ICE}$,
C.~E.~Cunha$^{\KIPAC}$,
L.~N.~da Costa$^{\LIneA,\ONR}$,
T.~de~Haan$^{\McGill,\Berkeley}$,
S.~Desai$^{\IITHyderabad}$,
H.~T.~Diehl$^{\FNAL}$,
J.~P.~Dietrich$^{\ExcellenceCluster,\LMU}$,
M.~A.~Dobbs$^{\McGill,\Cifar}$,
W.~B.~Everett$^{\Colorado}$,
E.~Fernandez$^{\IFAE}$,
B.~Flaugher$^{\FNAL}$,
J.~Frieman$^{\FNAL,\KICP}$,
J.~Garc\'ia-Bellido$^{\UAM}$,
E.~M.~George$^{\Berkeley,\ESO}$,
R.~A.~Gruendl$^{\Illast,\NCSA}$,
G.~Gutierrez$^{\FNAL}$,
N.~W.~Halverson$^{\Colorado,\Colphys}$,
N.~L.~Harrington$^{\Berkeley}$,
D.~L.~Hollowood$^{\SCIPP}$,
W.~L.~Holzapfel$^{\Berkeley}$,
K.~Honscheid$^{\CCAPP,\OSU}$,
J.~D.~Hrubes$^{\UChicago}$,
D.~J.~James$^{\CfA}$,
T.~Jeltema$^{\SCIPP}$,
K.~Kuehn$^{\AAO}$,
N.~Kuropatkin$^{\FNAL}$,
M.~Lima$^{\SaoPaulo,\LIneA}$,
H.~Lin$^{\FNAL}$,
A.~T.~Lee$^{\Berkeley,\LBNL}$,
E.~M.~Leitch$^{\KICPChicago,\AAUChicago}$,
D.~Luong-Van$^{\UChicago}$,
M.~A.~G.~Maia$^{\LIneA,\ONR}$,
D.~P.~Marrone$^{\Arizona}$,
J.~L.~Marshall$^{\TAMU}$,
P.~Martini$^{\CCAPP,\OSU}$,
J.~J.~McMahon$^{\Michigan}$,
P.~Melchior$^{\Princeton}$,
F.~Menanteau$^{\Illast,\NCSA}$,
S.~S.~Meyer$^{\KICPChicago,\AAUChicago,\EFIChicago,\PhysicsUChicago}$,
L.~M.~Mocanu$^{\KICPChicago,\AAUChicago}$,
J.~J.~Mohr$^{\Munich,\ExcellenceCluster,\MPE}$,
T.~Natoli$^{\KICPChicago,\PhysicsUChicago,\Dunlap}$,
R.~L.~C.~Ogando$^{\LIneA,\ONR}$,
S.~Padin$^{\KICPChicago,\AAUChicago}$,
A.~A.~Plazas$^{\JPL}$,
C.~Pryke$^{\Minnesota}$,
C.~L.~Reichardt$^{\Melbourne}$,
A.~K.~Romer$^{\Sussex}$,
A.~Roodman$^{\KIPAC,\SLAC}$,
J.~E.~Ruhl$^{\CaseWestern}$,
E.~S.~Rykoff$^{\KIPAC,\SLAC}$,
E.~Sanchez$^{\CIEMAT}$,
J.~T.~Sayre$^{\CaseWestern,\Colorado}$,
V.~Scarpine$^{\FNAL}$,
K.~K.~Schaffer$^{\KICPChicago,\EFIChicago,\ArtInstChicago}$,
R.~Schindler$^{\SLAC}$,
I.~Sevilla-Noarbe$^{\CIEMAT}$,
E.~Shirokoff$^{\Berkeley,\KICPChicago,\AAUChicago}$,
M.~Smith$^{\Southampton}$,
R.~C.~Smith$^{\CTIO}$,
M.~Soares-Santos$^{\Brandeis}$,
F.~Sobreira$^{\IFGW,\LIneA}$,
Z.~Staniszewski$^{\CaseWestern,\JPL}$,
A.~A.~Stark$^{\CfA}$,
E.~Suchyta$^{\ORNL}$,
M.~E.~C.~Swanson$^{\NCSA}$,
G.~Tarle$^{\Michigan}$,
D.~Thomas$^{\Portsmouth}$,
K.~Vanderlinde$^{\Dunlap,\UToronto}$,
J.~D.~Vieira$^{\Illast,\Illphys}$,
V.~Vikram$^{\ANL}$,
A.~R.~Walker$^{\CTIO}$,
J.~Weller$^{\ExcellenceCluster,\MPE,\LMU}$,
R.~Williamson$^{\KICPChicago,\AAUChicago}$
}
\vspace{0.4cm} \\
\parbox{\textwidth}{Author affiliations are listed at the end of this paper}}


